Data-Free Quantization Through Weight Equalization and Bias Correction

We introduce a data-free quantization method for deep neural networks that does not require fine-tuning or hyperparameter selection. It achieves near-original model performance on common computer vision architectures and tasks. 8-bit fixed-point quantization is essential for efficient inference on modern deep learning hardware. However, quantizing models to run in 8-bit is a non-trivial task, frequently leading to either significant performance reduction or engineering time spent on training a network to be amenable to quantization. Our approach relies on equalizing the weight ranges in the network by making use of a scale-equivariance property of activation functions. In addition the method corrects biases in the error that are introduced during quantization. This improves quantization accuracy performance, and can be applied to many common computer vision architectures with a straight forward API call. For common architectures, such as the MobileNet family, we achieve state-of-the-art quantized model performance. We further show that the method also extends to other computer vision architectures and tasks such as semantic segmentation and object detection.

==> sections/introduction-messy.tex <==
In recent years, deep learning models have moved from research labs into the cloud and onto edge devices.
As a result, power consumption and latency of deep learning inference have become an important concern.
%: mobile OEMs want to prevent the batteries of their customer's phones from draining too quickly due to models running on their devices, and companies deploying deep learning models on their servers want to minimize their models' energy consumption.
%One can vastly reduce the energy consumption of deep learning methods by representing their weights and values as 8-bit integers (INT8) instead of the usual 32-bit floating point (FP32) values. % also by doing the computation in this, should put that in this sentence
% By quantizing a model's FP32 weights and activations and representing them using INT8, efficient INT8 operations can be used, 
% \paragraph{INT8 quantization of FP32 models}
By quantizing FP32 values onto a regularly spaced grid, the original FP32 values can be approximated by a set of integers, a scaling factor, and an optional zero point offset \cite{jacob2018cvpr}.
This allows for the use of more efficient INT8 operations instead of FP32 operations in matmul or convolution computations, resulting in reduced energy consumption and lower latency at the expense of lower representational power.
% \todo{INT8 quantization only improves efficiency if the scaling factor and (optional) zero point are shared by a large number of values.
% For this reason, when quantizing a neural network, each tensor has its own set of quantization parameters, which is used to quantize all values in the tensor.
% For weight matrices, per-channel quantization is sometimes applied, in which each channel in a (convolutional) weight tensor has its own set of quantization parameters.
% This method however is not supported by all hardware.}
We refer the reader to \cite{jacob2018cvpr} for details on commonly used, hardware-friendly quantization methods for deep learning models.

% Given an FP32 value $x$, a scaling factor $\Delta$, and an integer offset $z$, the INT8 representation $x_{int}$ to $x$ can be found by:

% \begin{equation}
%     x_{int}=\text{round}\left(\frac{x}{\Delta}\right)+z
% \end{equation}
% where $x_{int}$ and $z$ are integers clipped to the range $[0, 127]$ for 8 bit quantization\footnote{This definition holds more generally for $N$-bit quantization, although for quantization to very low bit widths different quantization methods are generally used.}.
% The quantized FP32 approximation $\widetilde{x}$ can be computed as:
% \begin{equation}
%     \widetilde{x}=\Delta(x_{int}-z)
% \end{equation}

% When applying quantization to deep learning models, a different set of quantization parameters $\Delta$ and $z$ is used for each (weight and activation) tensor.
% Performing a matmul operation between two quantized matrices then requires only one FP32 operation which can be factored out of the matmul operation and applied when quantizing the output tensor.

% Per-channel quantization, in which the each output channel in a weight tensor has its own quantization parameters, has been proposed in the literature (e.g. \cite{krishnamoorthi}).
% However this method is not as widely supported by currently available hardware as per-tensor quantization.

% The $\Delta$ and $z$ quantization parameters for a tensor $\textbf{A}$ can be found as follows:

% \begin{align}
%     \Delta &= \frac{\max \textbf{A} - \min \textbf{A}}{2^N-1} \\
%     z &= \text{round}\left(\frac{-\min \textbf{A}}{\Delta} \right)
% \end{align}

% Multiplying two quantized values $\widetilde{x}_a$ and $\widetilde{x}_b$, with scaling factors $\Delta_a, \Delta_b$ and zero-point offsets $z_a, z_b$ then reduces to a set of integer multiplications and one FP32 multiplication:

% \begin{align}
%     \widetilde{x}_a\widetilde{x}_b &= \Delta_a\Delta_b(x_{int,a}x_{int,b}-z_ax_{int,b}-z_bx_{int,a}+z_az_b)
% \end{align}
% If this method is applied to a matrix operation, where each matrix has its own quantization parameters $\Delta$ and $z$, the products $\Delta_a\Delta$ and $z_az_b$ can be precomputed. The remaining products are INT8 operations. The matrix multiplication results in a new INT8 quantized matrix.

% Asymmetric quantization applied to tensors of values in a neural network, i.e. weight and quantization tensors, is available for 
% In this paper we focus on asymmetric per-tensor quantization. 
% When specialized hardware is used, multiplications between vectors FP32 values then reduce to INT8 vector multiplication and one FP32 scalar multiplication. 

% adding 'solutions' here makes sense, as the levels pertain to solutions, not the quantization

Quantization of FP32 models into INT8 introduces quantization noise on the weights and activations which often leads to reduced model performance. 
This reduction ranges from very minor to catastrophic.
For example, Krishnamoorthi \cite{krishnamoorthi} has recently shown that, for the image classification task, a wide range of pre-trained FP32 models can be quantized to INT8 with negligible loss in performance, but report complete loss of performance when quantizing the pre-trained Mobilenet \cite{} family of models .
% However, quantization destroyed performance of MobileNet family models, and fine-tuning was required to reach acceptable quantized performance. %post-training is a qualcommigism, not something general to distinguish between post and pre-training. 
The author was able to restore quantized performance to acceptable levels  on all models after performing fine-tuning. 
%or by employing quantization methods that are not supported on all currently available hardware.
% Quantized representations? % T: This feels a bit weird to me, what does this mean?

% There are many different ways of transforming a FP32 model to an INT8 model. 
% Many such methods rely on fine-tuning or training a model from scratch with quantization in mind.
\begin{figure}[t]
\includegraphics[width=8cm]{figures/imagenet_comparison.pdf}
\centering
\caption{Fixed point inference for MobileNet v2 on ImageNet. The original model has significant drop in performance from 12 bits whereas our model maintains close to FP32 performance until 6 bit.
% \todo{We need to somewhere reference to our plot. Otherwise it is kind of odd to have it here on page one.} 
}
\label{fig:imagenet_comparison}
\end{figure}

Methods introduced in the literature (e.g. \cite{jacob2018cvpr}, \cite{krishnamoorthi}) for mitigating the effect of quantization noise when quantizing existing FP32 models to INT8, often rely on quantization-aware fine-tuning or (re)training. 
These quantization processes are not always feasible in practice as a result of the data and computational requirements for fine-tuning or training. 
% In some cases they might not even be feasible due to time-constraints or problems with data-accessibility.
% We consider cases where the owner of the inference hardware is not in control of the model designing and training process. 
% This happens for example for cloud-services for inference that run deep-learning models, 
Real world actors for whom the traditional quantization processes are impractical include cloud-based deep learning inference service providers or cell-phone manufacturers that allow users to deploy models to their devices. 
For such stakeholders it would be preferable if FP32 models could be converted to INT8 without needing the know-how, data or compute necessary for running traditional quantization processes. %user's knowledge or effort explicitly. 
% A service that does the quantization on the fly, without needing data or retraining would be far more scalable and easy to use. 
Furthermore, quantization processes that do not use any data circumvent problems with privacy and ownership of data, and methods that do not require fine-tuning pave the way for easy-to-use and scalable quantization. 

% For example, fine-tuning a quantized model to a mobile device or the cloud might not be possible if the original data is not available, and not all hardware supports the quantized representations that perform well in experiments.
% For example, in the situation where a customer deploys their model to the cloud or a mobile device, it can't always be expected that the models' developer has the capability or time to make sure that their neural network functions well in 8-bits.
%For example, \cite{krishnamoorthi} shows that the popular MobileNetV2 architecture can only be quantized to INT8 if the model is fine-tuned after quantization; quantization 'out-of-the-box' results in a completely destroyed performance.
%However, the resources and data required for fine-tuning might not be available in all situations.
%In these cases it would be preferable to have a method that results in good quantized performance without requiring a training pipeline, a large computational budget, or extensive developer involvement.



\paragraph{Levels of quantization solutions}
To distinguish between the differences in applicability of quantization methods, we introduce four levels of quantization solutions, in decreasing order of practical applicability.
The axes for comparison are whether or not a method requires data, whether or not a method requires error backpropagation on the quantized model, and whether or not a method is generally applicable or requires significant model re-working.
% The axes for comparison
% \begin{itemize}
%     \setlength\itemsep{-0.2em}
%     \item Data: Whether a method requires data.
%     \item Backprop: Whether a method requires backprop.
%     \item Generality: Whether a method is applicable to any deep learning model.
% \end{itemize}

% For practical purposes, not all solutions to the quantization problem are created equal. For example, in a cloud or mobile setting where customers can deploy their neural network models, it can't always be expected that the developer of the model has the capability or time to make sure that their neural networks function well in 8-bits. A solution that quantizes a model to 8-bits without extra effort is much preferred. In our experience, we've also seen that not all models can be easily quantized and fine-tuned by introducing simulation ops as in \cite{jacob2018cvpr}, as the pre-fine-tuning accuracy is too low to start with. Thus to help assess the applicability and ease of use of quantization solutions for different use-cases, we introduce the following scheme. 


\begin{description}
    \item[Level 1] 
    No data and no backprop required. Works for any model.
    % Quantization can be done with an API call and works out-of-the-box.
    \item[Level 2] 
    Requires data but no backprop. Works for any model.
    The data is used e.g. to determine activation distributions, and to compute layer-wise loss functions. 
    However no fine-tuning pipeline, knowledge of the task or developer involvement is required.
    \item[Level 3] 
    Requires data and backprop. Works for any model.
    Model can be quantized but needs fine-tuning to reach acceptable performance. 
    These methods require a full training pipeline. (e.g. \cite{jacob2018cvpr} or \cite{krishnamoorthi})
    \item[Level 4] 
    Requires data and backprop. Only works for specific models.
    In this case, the network architecture needs non-trivial reworking, and/or the architecture needs to be trained from scratch with quantization in mind (e.g. \cite{sheng2018}, \cite{louizos2018relaxed}). 
    % This scenario is the least desirable, as the inference device provider would have to tell the customer to train a model entirely different from what they optimized before.
\end{description}


% The word performance is used too often



% \todo{fix first sentence}
In this paper, we argue that the distribution of values in weight tensors, specifically differences in distributions between output channels, causes model performance to drop after quantization.
Furthermore, we show that the quantization error on the weights can be biased.
We introduce a level 1 method that equalizes distributions within weight tensors to ease quantization, and corrects for the biased quantization error.
Lastly, we extend our method to compute activation distributions, which obviates the need to estimate activation ranges from data.
% In this paper, we show that some FP32 models require level 3 or level 4 approaches to quantize INT8 without significant loss in performance due to the distribution of their FP32 weights, and due to bias introduced by the quantization.
% In the next section we will illustrate the extent of this problem.
% Shouldn't we actually describe and visualize that problem here? This is the place to do it I think.
% We introduce a level 1 method that rescales the weight distributions across layers such that the model output is not affected, while making the weight distributions more amenable to quantization.
% We furthermore introduce a level 1 method that corrects for the bias introduced by quantization by updating the Batch Normalization statistics.
Applying these methods requires little to no developer input and no data.
We show that our method, when applied to a range of different models and tasks gives improved performance compared to the baseline.

% fine-tuning lot of work/hyper-parameter tuning, expensive.

% something for inference

% The focus of our paper is on quantization for inference. 

% Something on Mobilenet + describing the actual problem with quantization that we tackle

% Mention that per-channel quantization subsumes this. Also mention that the method works with partially linear 


% The only restrictions to the model that this can be applied to is that it needs to have piece-wise linear activation functions - 


% \idea{Shall we stress more 'quantization in the wild'? (i.e. no one does anything beyond  imagenet/MNIST)}

\paragraph{Contributions} This paper contains the following contributions.
\begin{itemize}
    \item We define levels of applicability for quantization methods.
    \item We introduce level 1 methods that enable post training quantization for many models that were previously found to be difficult to quantize.
    \item 
\end{itemize}



==> tables/exp1_bitwidths.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l r r}
        \toprule
        Bit-width & MobileNetV2 & MobileNetV2 + DFQ \\\midrule
        FP32      & 71.72\%     & 71.57\%\\
        INT16     & 71.72\%     & 71.60\%\\
        INT12     & 67.06\%     & 71.61\%\\
        INT10     & 2.28\%      & 71.53\%\\
        INT8      & 0.08\%      & 71.19\%\\
        INT6      & 0.10\%      & 64.12\%\\
        \bottomrule \\ \vspace{-.6cm}
    \end{tabular}
    \caption{Top1 ImageNet validation set results for MobileNetV2, evaluated at full precision different bit-widths.}
    \label{tbl:exp1_bitwidth}
\end{table}

